New optimal linear codes over $\ZZ_4$

In this work, we present novel approaches for constructing linear codes over $\ZZ_4$ from the known ones. We succeeded in obtaining new linear codes, many of which are optimal. In particular, we found all optimal codes for $k_1=2,~k_2=0$ and many optimal codes for $k_1=3,~k_2=0.$

==> tabel.tex <==
\begin{table*}[b]
\centering
\caption{New Plotkin-Optimal and Good Linear Codes for $k_1=2,k_2=0,2\leq n\leq 61$}
\label{tab1}\tabcolsep2.0pt\renewcommand{\arraystretch}{0.7}
\begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|c||c|c|c|c|c|c||c|c|c|c|c|c|}
	\hline
	n & Note &DB & Good & PLDB & LDB & n & Note &DB & Good & PLDB & LDB &n & Note &DB & Good & PLDB & LDB &n & Note &DB & Good & PLDB & LDB \\
	\hline
	2 &Known \cite{Aydin2}& 1  & 1      & 2  & 1
	&\textbf{17} &\textbf{L \ref{konstruk1}} & \textbf{16} & \textbf{17} & \textbf{18} & \textbf{31}
	&\textbf{32}&\textbf{L \ref{konstruk1}} &\textbf{32} & \textbf{33} & \textbf{34} & \textbf{61}
	&\textbf{47} &\textbf{L \ref{konstruk1}}& \textbf{48} & \textbf{49} & \textbf{50} & \textbf{91}  \\
	\hline
	3 &Known \cite{Aydin2}& 2  & 2      & 3  & 3
	&\textbf{18} &\textbf{L \ref{konstruk1}} & \textbf{17} & \textbf{18} &\textbf{19} &\textbf{33}
	&33 &L \ref{konstruk1} &34 & 34     & 35 & 63
	&\textbf{48} &\textbf{L \ref{konstruk1}}& \textbf{48} & \textbf{50} & \textbf{51} & \textbf{93} \\
	\hline
	\textbf{\textit{4}} &\textbf{\textit{Known \cite{Aydin2}}}& \textbf{\textit{4}}  & \textbf{\textit{4}}    & \textbf{\textit{4}}  & \textbf{\textit{5}}
	&\textbf{\textit{19}} &\textbf{\textit{\textbf{\textit{C \ref{opt1}}}}} &\textbf{\textit{18}} & \textbf{\textit{20}} &\textbf{\textit{20}} & \textbf{\textit{35}}
	&\textbf{\textit{34}} &\textbf{\textit{C \ref{opt1}}}&\textbf{\textit{34}} &\textbf{\textit{36}} & \textbf{\textit{36}} & \textbf{\textit{65}}
	&\textbf{\textit{49}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{50}} & \textbf{\textit{52}} & \textbf{\textit{52}} & \textbf{\textit{95}}\\
	\hline
	5 &Known \cite{Aydin2}& 4  & 4      & 5  & 7
	&20 &L \ref{konstruk1} & 20 & 20     & 21 & 37
	&35 &L \ref{konstruk1} & 36 & 36     & 37 & 67
	&\textbf{50} &\textbf{L \ref{konstruk1}} & \textbf{50} & \textbf{52} & \textbf{53} & \textbf{97}  \\
	\hline
	\textbf{\textit{6}} &\textbf{\textit{Known \cite{Dougherty2007}}} & \textbf{\textit{5}} & \textbf{\textit{6}}  & \textbf{\textit{6}}  & \textbf{\textit{9}}
	&\textbf{\textit{21}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{20}} & \textbf{\textit{22}} & \textbf{\textit{22}} & \textbf{\textit{39}}
	& \textbf{\textit{36}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{36}} & \textbf{\textit{38}} & \textbf{\textit{38}} & \textbf{\textit{69}}
	&\textbf{\textit{51}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{52}} & \textbf{\textit{54}} & \textbf{\textit{54}} & \textbf{\textit{99}}  \\
	\hline
	7 &L \ref{konstruk1} & 6  & 6      & 7  & 11
	&\textbf{22} &\textbf{L \ref{konstruk1}} & \textbf{21} & \textbf{22} & \textbf{23} & \textbf{41}
	&37 &L \ref{konstruk1} & 38 & 38     & 39 & 71
	&\textbf{52} &\textbf{L \ref{konstruk1}} & \textbf{52} & \textbf{54} & \textbf{55} & \textbf{101}\\
	
	\hline
	\textbf{\textit{8}} &\textbf{\textit{C \ref{opt2}}} & \textbf{\textit{8}}  & \textbf{\textit{8}} & \textbf{\textit{8}}  & \textbf{\textit{13}}
	&\textbf{\textit{23} }&\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{22}} & \textbf{\textit{24}} & \textbf{\textit{24}} & \textbf{\textit{43}}
	& \textbf{\textit{38}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{38}} & \textbf{\textit{40}} & \textbf{\textit{40}} & \textbf{\textit{73}}
	&\textbf{\textit{53}} &\textbf{\textit{C \ref{opt1}}} & \textbf{\textit{54}} & \textbf{\textit{56}} & \textbf{\textit{56}} & \textbf{\textit{103}}\\
	\hline
	9 &L \ref{konstruk1} & 8  & 8      & 9  & 15
	&24 &L \ref{konstruk1} & 24 & 24     & 25 & 45
	&39 &L \ref{konstruk1} & 40 & 40     & 41 & 75
	&\textbf{54} &\textbf{L \ref{konstruk1}} & \textbf{54}& \textbf{56} & \textbf{57} & \textbf{105} \\
	\hline
	\textbf{\textit{10}} &\textbf{\textit{C \ref{opt2}}} & \textbf{\textit{9}}  & \textbf{\textit{10}} & \textbf{\textit{10}}  & \textbf{\textit{17}}
	&\textbf{\textit{25}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{24}} & \textbf{\textit{26}} & \textbf{\textit{26}} & \textbf{\textit{47}}
	&\textbf{\textit{40}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{40}} & \textbf{\textit{42}} & \textbf{\textit{42}} & \textbf{\textit{77}}
	&\textbf{\textit{55}} &\textbf{\textit{C \ref{opt1}}} & \textbf{\textit{56}} & \textbf{\textit{58}} & \textbf{\textit{58}} & \textbf{\textit{107}}\\
	\hline
	11 &L \ref{konstruk1} & 10 & 10     & 11 & 19
	&\textbf{26} &\textbf{L \ref{konstruk1}} & \textbf{25}
	& \textbf{26} & \textbf{27} & \textbf{49}
	&41 &L \ref{konstruk1} &42 &42 &43 &79
	&\textbf{56} &\textbf{L \ref{konstruk1}}& \textbf{56} & \textbf{58} & \textbf{59} & \textbf{109} \\
	\hline
	\textbf{\textit{12}} &\textbf{\textit{C \ref{opt2}}} & \textbf{\textit{12}} & \textbf{\textit{12}} & \textbf{\textit{12}} & \textbf{\textit{21}}
	&\textbf{\textit{27}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{26}} & \textbf{\textit{28}} & \textbf{\textit{28}} & \textbf{\textit{51}}
	&\textbf{\textit{42}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{42}} & \textbf{\textit{44}} & \textbf{\textit{44}} & \textbf{\textit{81}}
	&\textbf{\textit{57}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{58}} & \textbf{\textit{60}} & \textbf{\textit{60}} & \textbf{\textit{111}} \\
	\hline
	\textit{\textbf{13}} &\textit{\textbf{\#}} & \textit{\textbf{12}} & \textit{\textbf{13}} & \textit{\textbf{13}} & \textit{\textbf{23}}
	&\textbf{\textit{28}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{28}}& \textbf{\textit{29}} & \textbf{\textit{29}} & \textbf{\textit{53}}
	&\textbf{\textit{43}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{44}} & \textbf{\textit{45}} & \textbf{\textit{45}} & \textbf{\textit{83}}
    &\textbf{\textit{58}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{60}} & \textbf{\textit{61}} & \textbf{\textit{61}} & \textbf{\textit{113}} \\
	\hline
	\textbf{\textit{14}} &\textbf{\textit{C \ref{opt2}}} & \textbf{\textit{13}} & \textbf{\textit{14}} & \textbf{\textit{14}} & \textbf{\textit{25}}
	&\textbf{\textit{29}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{30}} & \textbf{\textit{30}}     & \textbf{\textit{30}} & \textbf{\textit{55}}
	&\textbf{\textit{44}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{44}} & \textbf{\textit{46}} & \textbf{\textit{46}} & \textbf{\textit{85}}
	&\textbf{\textit{59}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{60}} & \textbf{\textit{62}} & \textbf{\textit{62}} & \textbf{\textit{115}} \\
	\hline
	\textbf{\textit{15}} &\textbf{\textit{T \ref{konstruk}}} & \textbf{\textit{14}} &
	\textbf{\textit{16}} & \textbf{\textit{16}} & \textbf{\textit{27}}
	&\textbf{\textit{30}} &\textbf{\textit{C \ref{opt1}}} &\textbf{\textit{30}} & \textbf{\textit{32}} & \textbf{\textit{32}} & \textbf{\textit{57}}
	&\textbf{\textit{45}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{46}} & \textbf{\textit{48}} & \textbf{\textit{48}} & \textbf{\textit{87}}
	&\textbf{\textit{60}} &\textbf{\textit{C \ref{opt1}}}& \textbf{\textit{62}} & \textbf{\textit{64}} & \textbf{\textit{64}} & \textbf{\textit{117}} \\
	\hline
	16 &\# & 16 & 16     & 17 & 29
	&31 &L \ref{konstruk1} & 32 & 32     & 33 & 59
	&46 &L \ref{konstruk1}& 46 & 48 & 49 & 89
	&61 &L \ref{konstruk1} & 64 & 64     & 65 & 119\\
	\hline
	
\end{tabular}
\vspace{-1.75ex}
{\textcolor{white}{(space)}\\DB: Database \cite{Aydin2}, C: Corollary, T: Theorem, L: Lemma, PLDB: Plotkin Lee Distance Bound (\ref{PLDB}), LDB: Lee Distance Bound (\ref{LDB1}), \textbf{\textit{bold-italic text:}} Plotkin-optimal,
\textbf{bolded text}: New good linear code, \#: Constructed by adding or deleting column(s) from the
generator matrix of the nearest optimal code.\par}
\end{table*}
